Semi-Autoregressive Energy Flows: Exploring Likelihood-Free Training of Normalizing Flows

Training normalizing flow generative models can be challenging due to the need to calculate computationally expensive determinants of Jacobians. This paper studies the likelihood-free training of flows and proposes the energy objective, an alternative sample-based loss based on proper scoring rules. The energy objective is determinant-free and supports flexible model architectures that are not easily compatible with maximum likelihood training, including semi-autoregressive energy flows, a novel model family that interpolates between fully autoregressive and non-autoregressive models. Energy flows feature competitive sample quality, posterior inference, and generation speed relative to likelihood-based flows; this performance is decorrelated from the quality of log-likelihood estimates, which are generally very poor. Our findings question the use of maximum likelihood as an objective or a metric, and contribute to a scientific study of its role in generative modeling.

==> reproducibility.tex <==
\section{Reproducibility}
\paragraph{Datasets} All datasets that we use are open-source. We have described in detail the datasets used in our experiments. The UCI dataset is used without preprocessing, and the digits and MNIST datasets are cast to floats and scaled to [0, 1] range from their original range.
\paragraph{Models} For each of our baselines as well as the main code, we have given implementational details in the Appendix \ref{sec:experimental} including layers, learning rate, and epochs. For our SAEF, we additionally provide a pseudocode in Appendix \ref{safpseudo}.
